Domain Generalization Emerges from Dreaming

Recent studies have proven that DNNs, unlike human vision, tend to exploit texture information rather than shape. Such texture bias is one of the factors for the poor generalization performance of DNNs. We observe that the texture bias negatively affects not only in-domain generalization but also out-of-distribution generalization, i.e., Domain Generalization. Motivated by the observation, we propose a new framework to reduce the texture bias of a model by a novel optimization-based data augmentation, dubbed Stylized Dream. Our framework utilizes adaptive instance normalization (AdaIN) to augment the style of an original image yet preserve the content. We then adopt a regularization loss to predict consistent outputs between Stylized Dream and original images, which encourages the model to learn shape-based representations. Extensive experiments show that the proposed method achieves state-of-the-art performance in out-of-distribution settings on public benchmark datasets: PACS, VLCS, OfficeHome, TerraIncognita, and DomainNet.

==> 3_Methods/3_2_Adversarial_Attack.tex <==
\subsubsection{Adversarial Attack and Defense}
\label{section:3.1.2}
Adversarial attacks aim to find the worst-case examples by searching for the artificial noise  that maximizes the loss with a certain constraint (\textit{e.g.,} $L_p$ norm balls).
Finding the adversarial examples can be defined as a numerical optimization problem below,
\begin{equation}
    \label{eq:adv_attack}
    \begin{split}
        &\max_\delta \mathcal L (x +\delta,\ y \ ; \theta) \\ 
        &\text{subject to } \delta \in \Delta,
    \end{split}
\end{equation}
where $\mathcal L$, $\theta$, and $\Delta$ denotes a training loss function, parameters of the model, and the feasible set of the noise respectively. 

Since Equation~\eqref {eq:adv_attack} is an NP-hard combinatorial problem~\cite{Belotti2013mixed}, no polynomial-time algorithm has been found yet to seek the global optimal solution. 
Instead, simple gradient-ascent-based  algorithms~\cite{goodfellow15fgsm,madry18pgd,carlini17cw} have been proposed to effectively find the adversarial examples. 
Specifically, an adversarial example which is iteratively estimated by projected gradient-ascent~\cite{madry18pgd} can be written as follows: 
\begin{equation}
    \label{eq:PGD}
    \begin{split}
        x^{i+1} &=  \Pi_{\Delta}\left ( x^i + \alpha \cdot \text{sign} (\nabla _{x^i} \mathcal L (x^i, y;\theta) \right ). \\ 
        %x &=  \Pi_{\Delta}\left ( x + alpha\ \cdot \text{sign} (\nabla _{x} \mathcal L (x, y;\theta) \right )
    \end{split}
\end{equation}
Here, $\Pi_{\Delta}$ denotes the projection function to the feasible set  $\Delta$. 
The solution of Equation~\eqref{eq:adv_attack} is approximated by updating Equation~\eqref{eq:PGD} with total $N$ iterations. 
During the iterations, $\theta$ is not updated to find the adversarial examples only dependent on the sample.

Adversarial training is one of the most common approaches to improve robustness against adversarial examples.
It is trained by minimizing the training loss estimated by the adversarial examples.
The adversarial training framework~\cite{madry18pgd} solves the following saddle point problem (min-max problem), which is composed of a non-convex outer minimization problem and a non-convex inner maximization problem:
\begin{equation}
    \label{eq:adv_train}
    \begin{split}
        &\min_\theta \max_{\delta \in \Delta} \mathbb E_{x \sim  \mathcal X , \ y \sim \mathcal Y}
        \left [ \  \mathcal L( x+\delta,\ y \ ; \theta)  
        \ \right ]
    \end{split}
\end{equation}
From Danskin’s theorem, if the loss function is continuously differentiable, gradients at inner maximizers correspond to the descent directions of the saddle point problem. 
In other words, we can solve Equation~\eqref{eq:adv_train} by independently generating adversarial examples first and feeding them for the model training. 
\input{Figures/main_figure}

==> 3_Methods/3_4_Adv_Training_copy.tex <==
\subsection{Training with Stylized Dream}
\label{sec:SDA_train}
We now present a learning strategy to train a network to predict consistent output between original images and \textit{Stylized Dream}.
Domain generalization aims to learn conditional distribution $P(Y|f(X))$ that is invariant to changes of the marginal distribution $P(X)$ across sources and target domains.
As aforementioned in Section~\ref{sec:intro}, we experimentally show that the model can generalize well on the unseen target domain when the model is trained to be less texture biased.
Motivated by the observation, we aim to make the feature extractor $f$ in $P(Y|f(X))$ to be independent of the textures.
% Motivated by the observation, our goal is to make the feature extractor $f$ in $P(Y|f(X))$ to be dependent on shapes rather than textures.
% To this end, we aim to make the shape-based representation be more informative than texture-based information.

For the purpose, the objective for training the network not to be texture biased can be formulated as follows: 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
    \label{eq:optimal}
    \begin{split}
        %\min_{f} \sum_{i=1}^{S} \sum_{j=S+1}^{S+T} \text{KL}\big ( P_j(Y|f(X))  \big \|  P_i(Y|f(X) \big ).
        \min_{f} \mathbb E \ \big [ D  \big (  P(Y|f(X_s^\prime)), \ P(Y|f(X_s)) \big )   \big ],
    \end{split}
\end{equation}
% \begin{equation}
%     \label{eq:optimal}
%     \begin{split}
%         %\min_{f} \sum_{i=1}^{S} \sum_{j=S+1}^{S+T} \text{KL}\big ( P_j(Y|f(X))  \big \|  P_i(Y|f(X) \big ).
%         \min_{f} \sum_{i < j} \mathbb{E} \ \big[ D  \big(  P_i(Y|f(X)), \ P_j(Y|f(X)) \big) \big],
%     \end{split}
% \end{equation}
where $D$ denotes the divergence metric between distributions, $X_s^\prime$ denotes a domain with more uninformative texture than sources $X_s$ (\textit{e.g.,} Stylized ImageNet).
% However, since the distribution of a target domain is unknown, we simulate the samples in the unseen domains by data augmentation.
Under the assumption that the less texture biased model generalizes better, $X_s^\prime$ emphasizes a specific inductive bias (\textit{i.e.,} shape-based representation) during training. 

Consequently, our goal is to make the output distribution of \textit{Stylized Dream} $p_\theta(y \ | \ x')$ consistent with the output distribution of source domains $p_\theta(y \ | \ x)$ where $p_\theta(y \ | \  x) = g(f(x))$.
Based on Equation~\eqref{eq:optimal}, our objective for consistency training can be formulated as follows: 
\begin{equation}
    \label{eq:consistency_reg}
    \begin{split}
        \min_{\theta} \ & \mathbb E_{x \sim \{  X_s \} _{s \neq t}, \ y \sim  Y} \big [\ D \left( p_\theta(y \ | \ x') ,\    p_\theta(y \ |\ x ) \right)\ \big] \\
        \text{  s.t. } & x' = x + \delta^* \\
        & \delta ^{*} = 
        \argmax_{\delta} \mathcal{L}_\text{dream} (x+\delta,\ \bar{x} \ ;f) ,
    \end{split}
\end{equation}
where $\bar{x}\neq x$ is an arbitrary image with the same label as $x$ to extract style for \textit{Stylized Dream}.
Equation~\eqref{eq:consistency_reg} makes the model less texture biased by matching the original images with the augmentations of uninformative texture.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Combining with a standard task-related supervised loss, our loss function can be rewritten as,
\begin{equation}
    \label{eq:training_loss}
    \begin{split}
        & \min_{f,\ g}  \ 
        \mathbb{E}_{x \sim \{  X_s \} _{s \neq t}, \ y \sim  Y} \left[ \  \mathcal{L}_{\text{ce}}(x,\ y \ ; f,g) 
        + D
        \big{(} g(f(x')) 
        ,\ g(f(x)) \big{)}  \ 
        \right] ,
        % \\ 
        % & \ \text{  s.t. } \delta ^{*} = 
        % \argmax_{\delta} \mathcal{L}_\text{dream} (x+\delta,\ \bar{x} \ ;f)
    \end{split}
\end{equation}
where $\mathcal L_{\text{ce}}$ denotes the cross-entropy loss for supervised learning.
Here, $\mathcal L_{\text{ce}}$ encourages the model to learn general representations from multiple source domains.

Similar to knowledge distillation, we use smoothed logits of the prediction (soft label) in training. Our final training loss function is written as,
\begin{equation}
    \label{eq:trades}
    \begin{split}
        &\min_\theta\mathbb E_{x, y} \bigg\{ \mathcal L_{\text{ce}} ( x,\ y \ ; \theta) +  \mathcal L_{\text{cons}} \big(\hat y^\prime / \tau,\ \hat y / \tau   \big)  
        \bigg\} ,
    \end{split}
\end{equation}
where $\mathcal L_{\text{cons}}$ is a consistency loss as a divergence metric, we use MSE loss, JS divergence, and KL divergence loss in experiments. 
$\hat y ^\prime$ and $\hat y $ denote a predicted logit of the \textit{Stylized Dream}  and original image, and $\tau$ denotes  temperature parameter. 
\input{Algorithms/Alg2}
Algorithm~\ref{alg:training} shows our training scheme with SD. \\

{
\noindent{\textit{\textbf{Remarks.}}}
Our framework is relevant to standard adversarial training in the sense that both methods generate augmented samples by numerical optimization schemes. 
However, adversarial training is different from our method in the two aspects. 
First, adversarial training generates the worst-case examples by maximizing the original supervised loss whereas our Stylized Dream (SD) 
generates an augmented sample by maximizing the activation of a stylized image, which is independent from the original loss.
%Secondly, since our framework does not focus on imperceptible noise, our augmentation is not limited to a small perturbation.
Second, our framework encourages the consistency between predictions on clean and augmented samples by consistency regularization whereas the adversarial training directly optimizes the original supervised loss with the augmented samples.
}


==> Figures/SD2.tex <==
\renewcommand\thefigure{3}
\begin{figure}[!t]
    \centering
    \caption{\textbf{Examples of Stlized Dream.} 
    Row (a) denotes the original image, row (b) denotes arbitrary target style image, (c) denotes the Stylized Dream image with ResNet-18, and row (c) denotes the Stylized Dream image with VGGNet-16.   
    All the Stylized Dream examples are visualized with 10 iterations and 0.09 of step size $\alpha$.
    Best viewed in color.
    }
    \vspace{5pt}
    \includegraphics[width=\columnwidth]{Figures/SD2_file.pdf}
    \label{fig:SD2}
\end{figure}

==> Tables/0_Main_copy.tex <==
\begin{table*}[htp]
    \centering
    \small
    %\setlength{\tabcolsep}{3pt}
    %\begin{adjustbox}{width=1\textwidth} 
    \caption{
    \textbf{Comparison with the state-of-the-art domain generalization methods and SDA on PACS dataset.} 
    All experiments are evaluated in out-of-distribution setting using ResNet-18 and ResNet-50 architectures. 
    The title of the each column indicates the test target domain.
    We report RSC*~\cite{Huang20RSC} as reproducible performance. DSON*~\cite{Seo20DSON} denotes DSON model with domain-specific mixture-weights, \textit{i.e.}, model ensemble performance. 
    \textbf{Bold} denotes the best performance.
    We report the average accuracy of three independent runs.}
    \label{tab:pacs}
    \begin{tabular}{l|c c c c|c} 
    \toprule
    \multicolumn{1}{l|}{\textbf{ Method}} & \multicolumn{1}{c}{$\ \ $Art Paint $\ $} & \multicolumn{1}{c}{$\ \ $ Cartoon $\ \ $} & \multicolumn{1}{c}{$\ \ $ Photo $\ \ $} & \multicolumn{1}{c|}{$\quad $  Sketch  $\quad $}& {\textbf{ Average (\%) }} \\  
    \hline \hline
    \rowcolor{Gray} 
    % 18 실험 
    \textbf{ResNet-18} &  &  &  &  & \\
    
    JiGen~\cite{Carlucci19jigen} 
    & 79.42 & 70.41 & 95.87 & 70.68 & 78.86 \\
    
    D-SAM~\cite{antonio18dsam} 
    & 77.33 & 72.43 & 95.30 & 77.83 & 80.72 \\
    
    MSAF~\cite{Dou19msaf} 
    & 80.29 & 77.17 & 94.99 & 71.69 & 81.04  \\
    
    ER~\cite{zhao20er}
    & 80.70 & 76.40 & \textbf{96.65} & 71.77 & 81.38 \\
    
    DMG~\cite{Chattopadhyay20DMG} 
    & 76.90 & \textbf{80.38}& 93.35 & 75.21  & 81.46 \\
    
    EpiFCR~\cite{Li19epifcr} 
    & 82.10 & 77.00 & 93.90 & 73.00 & 81.50   \\
    
    RSC*~\cite{Huang20RSC}
    & 78.90 & 76.88 & 94.10 & 76.81 & 81.67 \\
    
    MetaReg~\cite{Balaji18metareg} 
    & {83.70} & 77.20 & 95.50 & 70.30 & 81.70  \\
    
    MMLD~\cite{Matsuura20mmld} 
    & 81.28 & 77.16 & 96.09 & 72.29 & 81.83 \\
    
    EISNet~\cite{wang20eisnet} 
    & 81.89 & 76.44 & 95.93 & 74.33 & 82.15 \\
    
    I-Drop~\cite{shi20idrop} 
    & 80.27 & 76.54 & 96.11 & 76.38 & 82.32 \\
    
    pAdaIN~\cite{nuriel21padain} 
    & 81.74 & 76.91 & 96.29 & 75.13 & 82.51 \\
    
    SagNet~\cite{Nam21sagnet} 
    & 83.58 & 77.66 & 95.47 & 76.30 & 83.25 \\
    
    SelfReg~\cite{Kim21selfreg} 
    & 82.34 & 78.43 & 96.22 & {77.47} & {83.62} \\
    %$ ^{\dagger}$ \\
    
    MixStyle~\cite{zhou21mix} 
    & {84.1} & {78.8}& 96.1 & 75.9  & {83.7} \\
    
    L2D~\cite{wang2021l2d} 
    & 81.44 & 79.56  & 95.51 & {80.58} & {84.27} \\
    
    DSON~\cite{Seo20DSON} 
    & 82.13 & 74.10& 95.03 & {80.02} & 82.82 \\
    
    DSON*~\cite{Seo20DSON} & \textbf{84.67} & 77.65 & 95.87 & \textbf{82.23} & \textbf{85.11} \\
    \hline 
    
    
    \multirow{2}{*}{\textbf{Ours}$_\text{SDA}$}
    & 84.47
    & 78.92 
    & 95.75 
    & 77.98
    & 84.28 \\

    & ($\pm$0.17)
    & ($\pm$0.24)
    & ($\pm$0.11)
    & ($\pm$0.23)
    & ($\pm$0.44)\\
    
    \hline \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \rowcolor{Gray} \textbf{ResNet-50} &  &  &  &  & \\ 
    
    MetaReg~\cite{Balaji18metareg} 
    & 87.20  &  79.20  &  97.60 &  70.30 & 83.60 \\
    
    MSAF~\cite{Dou19msaf} 
    & 82.89 & 80.49 & 95.01 & 72.29 & 82.67 \\
    
    RSC*~\cite{Huang20RSC} 
    & 81.38 & 80.14 & 93.72 & 82.31 & 84.38 \\
    
    ER~\cite{zhao20er} 
    & {87.51} & 79.31 & \textbf{98.25} & 76.30 & 85.34  \\
    
    CORAL~\cite{sun2016coral} 
    & 88.30 & 80.00 & 97.50 & 78.80 & 86.20  \\
    
    ARM~\cite{zhang2020arm} 
    & 86.80 & 76.80 & 97.40 & 79.30 & 85.10  \\
    
    Mixup~\cite{yan2020mixup} 
    & 86.10 & 78.90 & 97.60 & 75.80 & 84.60  \\
    
    pAdaIN~\cite{nuriel21padain} 
    & 85.82 & 81.06 & 97.17 & 77.37 & 85.36 \\
    
    ERM~\cite{Gulrajani21domainbed} 
    & 84.70 & 80.80 & 97.20 & 79.30 & 85.50 \\
    
    EISNet~\cite{wang20eisnet} 
    & 86.64 & 81.53 & 97.11 & 78.07 & 85.84 \\
    
    DSON*~\cite{Seo20DSON} 
    & 87.04 & 80.62 & 95.99 & {82.90} & 86.64  \\
    
    SelfReg~\cite{Kim21selfreg} 
    & 87.90 & 79.40 & 96.80 & 78.30 & 85.60  \\
    
    SagNet~\cite{Nam21sagnet} 
    & 87.40 & 80.70 & 97.10 & 80.00 & 86.30  \\
    
    SWAD~\cite{cha2021swad}
    & {89.3} & {83.4} & 97.3 & 82.5 & {88.1} \\ 
    \hline
    %\multicolumn{1}{c|}{\textbf{Ours}
    % \multirow{2}{*}{\textbf{Ours}$_\text{SDA}$}
    % & \textbf{87.78} 
    % % Swa Test Acc: 87.89 
    
    % % Swa Test Acc: 87.55 
    % % Swa Test Acc: 87.89 
    % %                       88.08 (+- 0.25)  
    
    % & \textbf{82.82} 
    % % Swa Test Acc: 82.94 
    % % Swa Test Acc: 82.04 
    % % Swa Test Acc: 83.48 
    
    % & \textbf{81.95} 
    % % Swa Test Acc:81.94 
    % % Swa Test Acc:82.42 
    % % Swa Test Acc:81.46 
    
    % & \textbf{97.97}${}^\dagger$  
    % % Swa Test Acc:97.96 
    
    
    % & {\textbf{87.62}}  \\
    % % 88.18
    % % 88.00
    % % 88.20
    
    % & ($\pm$0.16)
    % & ($\pm$0.34)
    % & ($\pm$0.39)
    % & ($\pm$0.02)
    % & ($\pm$0.05) \\
    \multirow{2}{*}{\textbf{Ours}$_\text{SDA}$}
    % 83.96, 84.88, 90.23, 96.77
    & \textbf{90.23} 
    & \textbf{84.88} 
    & {96.77}
    & \textbf{83.96} 
    & {\textbf{88.96}}  \\
    
    & ($\pm$0.52)
    & ($\pm$0.24)
    & ($\pm$0.93)
    & ($\pm$0.05)
    & ($\pm$0.33) \\
    
    %{\textbf{Ours}$_\text{SDA+SWAD}$}
    % %90.09  84.64 96.69 82.86 88.57
    % %89.262%    | 83.422% | 97.081% | 83.524% | 88.322%
    %& {89.26}
    %& \textbf{83.42}
    %& {97.08}
    %& \textbf{83.52}
    %& \textbf{88.32} \\
    
    % &  &  &  &  &  &  \\
    \bottomrule
  \end{tabular}
  \vspace{3pt}
  %\end{adjustbox}
\end{table*}






==> Tables/4_AdaIN.tex <==
\begin{table}[hp]
    \small
    \centering
    \begin{tabular}{c c c c c c c}
        \toprule
        %\multirow{2}{*}{Model} & 
        \multicolumn{2}{c}{\textbf{SDA}} & \multicolumn{4}{c}{\textbf{Target Domain}} & \multirow{2}{*}{\textit{Average} (\%)}
        \\
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-6} 
        
        \textit{w AdaIN}
        & \textit{w/o AdaIN}
        & A %\textit{Art Painting}
        & C %\textit{$\ $Cartoon$\ $}
        & P %\textit{$\quad $Photo$\quad $}
        & S %\textit{$\ $Sketch$\ $}
        \\
        \midrule
        {}
        & \multicolumn{1}{c}{\checkmark }
        & {88.18} 
        & {79.86} 
        & \textbf{97.49} 
        & \multicolumn{1}{c}{78.34} & 85.97 \\
        
        \checkmark 
        & \multicolumn{1}{c}{} 
        & \textbf{89.45} 
        & \textbf{82.89} 
        & 97.17 
        & \multicolumn{1}{c}{\textbf{82.62}} 
        & \textbf{88.03} \\ 
        
        \bottomrule
    \end{tabular}
    \vspace{3pt}
    \caption{\textbf{Ablation study of SDA with and without AdaIN.} Average accuracy of SDA adversarial training on PACS datasets. 
    First and second rows denote SDA attack with and without AdaIN respectively. }
    \label{table:adain_ablation}
\end{table}

==> Tables/6_BagNets.tex <==
\begin{table*}[!ht]
  \centering
  \small
  \caption{\textbf{Out-of-distribution evaluation of BagNets on PACS.} 
  The title of each column indicates the test target domain. \textit{i.e.}, trained in other 3 domains and tested at target. Here, A, C, S, P denotes Art painting, Cartoon, Sketch, and Photo respectively.
  We also report the ResNet-50 and ResNet-18 performance for the comparison.
  BagNet-$N$ denotes BagNets with restricted receptive fields of $N \times N$ pixels.
  }
  \label{tab:bagnets}
  \begin{tabular}{ c  c c c c c}
    \toprule
    \multirow{2}{*}{$\quad$ \textbf{Model} $\quad$ } 
    & \multicolumn{4}{c}{$\quad$ \textbf{Target Domain} $\quad$}
    & \multirow{2}{*}{ \textit{Average}(\%) }
    \\
    
    \cmidrule{2-5}
     & {A} 
     & {C}
     & {S}
     & {P} \hspace{1pt} 
    \\ 
    
    \midrule
    
    ResNet-50
    & 85.16 
    & 78.89
    & 78.04 
    & 95.07
    & 84.29 
    \\
    
    ResNet-18
    & $\ $ 79.89 $\ $ 
    & $\ $ 75.61 $\ $
    & $\ $ 73.33 $\ $
    & $\ $ 95.66 $\ $
    & $\ $ 81.12 $\ $
    \\
    
    \midrule
    
    {BagNet-33} 
    & 62.79
    & 64.25
    & 34.69
    & 92.04
    & 63.44
    \\
    
    {BagNet-17} 
    & 50.68
    & 50.34
    & 24.76
    & 85.69
    & 52.87
    \\ 
    
    {BagNet-9}
    & 40.28 
    & 45.52 
    & 22.48 
    & 74.13 
    & 48.10
    \\ 
    
    {}
    & 
    & 
    & 
    &
    &
    \\
    
    \bottomrule
  \end{tabular}
\end{table*}


==> Tables/temp.tex <==
\begin{table*}[!ht]
  %The ground-truth of IMDB-M is calculated by Beam, Hungarian, and VJ. }
  \centering
  \small
  \caption{\textbf{Consistency Training with various regularization metric.} \textit{Abbr.} \textit{MSE} : Mean-Squared Error, \textit{KL Div.} KL-divergence. }
  \label{tab:divergence}
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{ c  c   c c c c  c  }
    % \begin{tabular}{ c  c c  c c c c  c  }

    \toprule
    \multirow{2}{*}{$\quad$  \textbf{Model}  $\quad$ } 
    % & \multicolumn{2}{c}{\textbf{Divergence Metric}}   
    & \multirow{2}{*}{$\quad$ \textbf{Divergence Metric}(\%) $\quad$}
    & \multicolumn{4}{c}{\textbf{Test Domain}} 
    & \multirow{2}{*}{$\quad$ \textit{Average}(\%) $\quad$}
    \\
    \cmidrule{2-3}
    \cmidrule{4-7} 
    %  & $\quad$ \textit{MSE} & \textit{KL Div.}
     &
     & {A} 
     & {C} 
     & {S} 
     & {P} \hspace{1pt} 
     \\  \midrule
    
    \multirow{2}{*}{ResNet-50}
    & $\quad $ \checkmark &
    & $\ $ 87.70 $\ $ 
    & $\ $ 82.76 $\ $ 
    & $\ $ 81.90 $\ $ 
    & \textbf{97.49} 
    & $\ $ 87.46 $\ $ 
    \\
     
        % & & \checkmark &

    &  \checkmark &
    \textbf{90.23}  & 
    \textbf{84.88}  & 
    \textbf{83.96}  & 
    $\ $ {96.77} $\ $  & 
    \textbf{88.96}  \\ 
    
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \vspace{3pt}
\end{table*}



